Cloudburst: Stateful Functions-as-a-Service

Function-as-a-Service (FaaS) platforms and "serverless" cloud computing are becoming increasingly popular. Current FaaS offerings are targeted at stateless functions that do minimal I/O and communication. We argue that the benefits of serverless computing can be extended to a broader range of applications and algorithms. We present the design and implementation of Cloudburst, a stateful FaaS platform that provides familiar Python programming with low-latency mutable state and communication, while maintaining the autoscaling benefits of serverless computing. Cloudburst accomplishes this by leveraging Anna, an autoscaling key-value store, for state sharing and overlay routing combined with mutable caches co-located with function executors for data locality. Performant cache consistency emerges as a key challenge in this architecture. To this end, Cloudburst provides a combination of lattice-encapsulated state and new definitions and protocols for distributed session consistency. Empirical results on benchmarks and diverse applications show that Cloudburst makes stateful functions practical, reducing the state-management overheads of current FaaS platforms by orders of magnitude while also improving the state of the art in serverless consistency.

==> tex/intro.tex <==
\section{Introduction} \label{sec:intro}

Serverless computing has attracted significant attention in recent years, with current interest focused on Function-as-a-Service (FaaS) platforms. 
Application developers are drawn to the ability to write code in traditional programming languages and easily deploy it in the cloud. 
Key benefits include minimal administrative burden and consumption-based pricing via transparent autoscaling of resources from zero to peak load and back.
Cloud providers benefit from the separation of computation and storage in serverless architectures, which enables them to achieve higher utilization at the infrastructure level because users' compute and storage can be separately packed and scaled in multitenanted environments.
These benefits have made FaaS platforms an attractive option for a variety of applications in both research and industry~\cite{excamera, pywren, akkus2018sand, bv-serverless, serverless-cidr19, pocket, baldini2017serverless, van2017spec, gan2019open, fouladi2019laptop, awscasestudies}.


Programming with functions is attractive in part because pure functional programming involves only local, immutable state.
Perhaps as a result, one of the architectural shortcomings of current FaaS platforms is that they provide very weak support for stateful programs, especially for mutable shared state. 
While state can be shared across function invocations, it is only possible via autoscaling storage services like AWS S3 and DynamoDB. 
These storage services have been shown to have latencies and operational costs that are orders of magnitude worse than standard infrastructure like shared memory, network protocols, or lightweight shared storage~\cite{wang2018peeking,serverless-cidr19}.

\vikram{I think the stuff about strong consistency goes here?}

The architectural shortcomings of FaaS state handling lead to significant practical problems for developers.
First, current FaaS platforms pay a high storage cost during basic function processing.
The arguments and return values in a nested function invocation are a form of communication---i.e., state-sharing---between parent and child functions. 
In current FaaS platforms, these function invocations require round-trips through expensive high-latency storage services ($\S$\ref{sec:eval-composition}), which discourages general-purpose functional programming with stack depths greater than one.

Second, despite the widespread discussion of ``lambdas,'' current FaaS platforms were never intended for pure functional programming: Mutable storage APIs are an integral part of all serverless offerings.
A majority of the commercial use cases touted by the vendors~\cite{awscasestudies} as well as serverless research applications~\cite{excamera,pywren,numpywren} make extensive use of storage services. 

Finally, it is quite common for scalable applications to use distributed resources and engage in low-latency communication between distributed processes.
Implementing communication via cloud storage is orders of magnitude slower in a system like S3 than via network protocols ($\S$\ref{sec:eval-comm}). 
This limits developers' ability to pursue general-purpose distributed applications in current FaaS platforms.

Of course, there are good reasons why first-generation FaaS platforms do not support mutable shared storage efficiently.
The first is the design pattern of disaggregating compute from storage.
\vikram{Copied from Joe's note in section 2: don't cut this motivation.}
A second reason is that shared mutable state leads to the known hard problems of distributed consistency being exposed to the programmer.
Most autoscaling cloud storage services---including the recommended solutions from AWS, Azure, and GCP---do not solve this problem; they provide weak eventual consistency guarantees.

In this paper, we present a new programmable serverless platform called \fullsystem{} that removes the shortcomings of commercial FaaS architectures highlighted above, without sacrificing their benefits.
The key contribution of \system{} is to solve the problem of providing low-latency mutable shared state across autoscaling invocations of general-purpose code, without exposing developers to inexplicable consistency bugs. \todo{Reframe this contribution.}

Networking and shared storage---both forms of cross-function state sharing---are supported by a combination of an autoscaling key-value store (KVS) and mutable KVS caches that are co-located with the function evaluators. 
The caches provide data locality, solving many of the latency problems of earlier FaaS architectures, while the KVS serves both as a backbone for efficient cross-function sharing of state and an overlay network for communication among logical endpoints in an autoscaling physical environment.

This leaves the thorny problem of consistency for mutable shared state across distributed function invocations. 
A particular challenge is that compositions of functions form a session~\cite{terry1994session} that migrates across multiple distributed locations. 
The caches in those locations may be out of sync even though each is locally consistent.
To address this concern, we develop novel \emph{transfunctional consistency} specifications and protocols, which ensure that all references to an object in a program---regardless of where they originate---observe a uniform consistency level.

We evaluate \system{} via microbenchmarks as well as two application scenarios using third-party code, demonstrating benefits in raw performance, predictable latency, and consistency. 
The contributions of this paper include:
\vspace{-0.1em}
\begin{enumerate}\itemsep0em
    \item The design and implementation of an autoscaling serverless architecture for stateful and distributed code written in a traditional programming language.

    \item Per-object cache consistency via \emph{lattice capsules}, which wrap program state in metadata that enables rich consistency to be maintained via simple KVS merge APIs.

    \item The identification of new \emph{transfunctional consistency} challenges in the distributed execution of functions, and protocols to ensure that compositions of functions observe consistent state regardless of where they run.

\end{enumerate}

% The first reason has become conventional wisdom in modern cloud systems: It is desirable to disaggregate computing from storage in the cloud~\cite{}. 
% Scaling compute separately from data allows systems---especially multiuser and multitenanted systems---to dynamically ``shape'' their resource mix to workload shifts over time. 
% In particular, compute resources can be scaled to zero during idle times (a major cost savings), without sacrificing the ability to easily scale back up as demand increases.
% As we will see empirically ($\S$\ref{sec:eval-consistency}), moving to more efficient latency regimes would quickly expose consistency problems to developers. 
% The current architectures mask their consistency weakness with high latency; solving the latter problem unmasks the former.

% We evaluate \system{} deployed on top of an autoscaling KVS called Anna~\cite{wu2019anna,anna-vldb} that offers low latency and supports extensible merge functions. 
% Microbenchmarks demonstrate that \system{} can achieve orders of magnitude improvements over the current major FaaS offerings for basic tasks like simple function invocation and composition, with low-latency shared storage access and cross-functional communication. 
% We show that the overhead of choosing richer consistency is typically quite modest relative to microbenchmark baselines.
% % and even 99th percentile performance levels for causal consistency in \system{} outperforms median performance of competing FaaS services with best-effort eventual consistency. 
% We demonstrate the autoscaling ability of \system{}, and present two scenarios that demonstrate the performance of \system{} in relatively full-featured applications. 
% In the first, we show how off-the-shelf code for prediction serving~\cite{clipper-nsdi17,tf-serving} using PyTorch~\cite{} can be easily launched over \system{} and provide performance that is both faster and more predictable than AWS Sagemaker, a bespoke cloud service for that domain.
% In the second, we port a frequently-studied Python based Twitter clone called ReTwis~\cite{retwis}, which relies on causal consistency to work properly, showing that \jmh{... finish me.}

% To address this, \system{} uses a coordination-free approach that provides transparent distributed cache consistency. 
% Building on prior work~\cite{Bailis:2013:BCC:2463676.2465279,Conway:2012:LLD:2391229.2391230,wu2019anna}, \system{}'s caches wrap program state in \emph{lattice capsules}, which allow arbitrary cache updates to be merged consistently in any order via associative, commutative and idempotent \texttt{merge} functions. 
% % Lattice capsules can be used over any KVS that supports user-defined merge (conflict resolution) functions, providing bolt-on per-object consistency levels up to and including causal consistency.
% We observe, however, that reorderable updates alone are not sufficient to ensure consistency for serverless computing. 

% Serverless computing  % have generated increasing interest recently because they 
% offers a computing platform with an attractive combination of features, including fine-grained autoscaling, minimal operational overhead, and a pay-as-you-go billing model. 
% Cloud vendors have begun offering backend services with serverless features (e.g. AWS Athena and Google Cloud Dataflow), but these typically provide developers with limited data-centric DSLs for programming (SQL or map-reduce-style dataflow). 
% To complement these Backend-as-a-Service (BaaS) offerings, the cloud vendors also offer more flexibly-programmable Function-as-a-Service (FaaS) offerings like AWS Lambda, Google Cloud Functions and Azure Functions. 
% These services allow programmers to write arbitrary functions in familiar languages like Python, Go or JavaScript, and very easily deploy them in the cloud to respond to requests on demand in an autoscaling fashion.
% \jss{lots of business / industry speak in here. How do we get a SOSP reviewer hooked and wanting to read more?}

% FaaS has generated excitement among both researchers and production customers with a breadth of compelling use cases~\cite{}. 
% But the limitations of FaaS offerings have also been well documented~\cite{}. 
% Chief among these limitations are (1) the high latency of data transfer into and out of functions, and (2) the inability for functions to communicate via point-to-point messaging. 
% In essence, the current FaaS offerings achieve autoscaling by ensuring that functions are largely \emph{stateless}: they can only be contacted via invocation, and do not retain any state across invocations. 
% The only way for state to be persisted and/or communicated across functions is to use high-latency storage systems: e.g. S3 or DynamoDB in the AWS ecosystem. 

% Stateless functions make basic efficiency patterns like data locality, session affinity and even simple message-passing impossible or expensive in current serverless frameworks. 
% For many application scenarios this can lead to orders of magnitude overheads in latency and cost relative to traditional ``serverful'' designs~\cite{}. \jmh{Moreover, the BaaS storage offered to most serverless functions today provide weak consistency, which means that chains of functions that write to storage may observe inconsistent state.}

% In response to the limitations of current FaaS offerings, it is natural to consider designing a \emph{stateful serverless} platform that allows network-addressable code to be colocated with mutable state.  
% The idea of stateful serverless computing raises a number of technical challenges that need to be overcome:

% \begin{enumerate}
%     \item \textbf{Autoscaling without sacrifices.} Current serverless offerings provide autoscaling, but only with high-latency and expensive data access and communication. 
%     Can we achieve a general-purpose data-rich programming interface that offers autoscaling, low latency access to data, and fine-grained communication?
%     \item \textbf{Logical separation, physical colocation.} A desirable and common design pattern in autoscaling cloud computing is the separation of storage and compute tiers, allowing each to scale up or down independently of the other. 
%     Today this is typically done by physically separating the tiers, which leads to stateless computing with high-latency access to storage. 
%     Can we separate compute and storage resource allocation, yet still achieve physical co-location of compute and storage as needed?
%     \item \textbf{Autoscaling with program consistency.} Statelessness sidesteps many of the classical challenges of distributed computing, which revolve around the consistency of state. 
%     Yet traditional solutions to distributed programming typically rely on transactions or other mechanisms requiring quora of replicated state machines with slowly-changing membership~\cite{}. 
%     If we allow arbitrary user code to be both stateful and autoscaling, can we achieve rich consistency without fixed server?
% \end{enumerate}

% The contributions of the work include the following:
% \begin{itemize}
% \item The design and implementation of \system{}'s serverless runtime, which enables the development of performant, stateful programs with independent autoscaling of compute and storage. 
%     % The runtime guarantees atomic execution of chains of functions and achieves high performance by minimizing data movement and applying caching. 
% \item \emph{Lattice-tagged cache consistency}, which allows general-purpose, mutable programming-language objects to be co-located with autoscaling functions, while still ensuring rich consistency.
% \item A new \emph{cross-function causal consistency} technique, which ensures that programs can achieve causal consistency across function invocations as well as I/Os.
% \item An evaluation of \system{} relative to the leading FaaS framework today, AWS Lambda. The evaluation includes metrics from microbenchmarks comparing \system{} to AWS Lambda with regard to X, Y and Z. It also includes a report on our implementation of two applications that demonstrate the simplicity of deploying code in \system{}. These include an open-source version of Twitter called retwis \todo{cite}, and a low-latency machine learning model serving system in the spirit of Tensorflow Serving~\cite{} and Clipper~\cite{}.
% \end{itemize}

==> tex/responses.tex <==
\newcommand{\response}[1]{{\color{blue}#1}}

\newcommand{\review}[1]{{\color{black}#1}}

\begin{center}
\begin{LARGE}
{\bf Overview of Edits Based on Reviewer Feedback}
\end{LARGE}
\end{center}

We thank the reviewers for their careful reading of our paper and helpful comments on how to improve it.  
We have revised the paper based on the comments and believe that the work significantly benefited from the feedback. 

Our revision includes a number of significant changes.
First, we expanded the discussion of the semantics and functionality of a number of core features of \system{}, especially message passing and causal consistency.
We added detailed descriptions of how both features work and described the metadata associated with causal consistency.
We also demonstrated the scalability of the system by increasing the size of the autoscaling experiment and measuring key overheads (cached key index and causal metadata sizes).

In addition, we used the feedback to clarify the exposition in the paper. 
Below we address all of the suggestions from the reviewers in detail and point out where the changes can be found in the new version of the paper.
We have highlighted the changes we have made to the paper in blue font.

\begin{LARGE}
\textbf{\\ Response to Reviewer 2 \\}
\end{LARGE}

\review{\noindent \textbf{R1.} Address W1. Does W1 significantly restrict cloudburst's usefulness?
The authors should also discuss the differences between function decomposition into DAGs as in Cloudburst, and chaining functions, as in AWS.\\}

\response{\noindent 
% \chenggang{I think in the first sentence we should state clearly that we do NOT require functions to declare the reference ahead of time.
% And flip the order of the following two sentences.}

\system{} does not require that functions always pre-declare their data accesses before execution.
Functions that need to dynamically retrieve data can do so using the communication API described in Section~\ref{sec:programming}---we clarified this in the text in that section.
However, you are correct that requests requiring locality must include references to data accesses up front.
There are techniques from the programming languages community (e.g., continuations) that would allow users to automatically take advantage of locality by splitting requests around IOs, but those techniques are out of scope for this paper.

While the APIs for function decomposition and function chaining in AWS differ, the goals and functionality are similar: moving results from one function to the next.
As we demonstrate in the evaluation, Cloudburst's model of pre-declaring DAGs leads to significant performance wins.
We have clarified this point as well in Section~\ref{sec:programming}.
\\}

\review{\noindent \textbf{R2.} The authors should compare Cloudburst to its competitors using a stateless application. (this is W3 above)\\}

\response{\noindent 
Thanks for this suggestion.
To evaluate a stateless application, we extended the experiment in Section~\ref{sec:eval-compostition} to include a single function invocation in addition to function compositions.
Cloudburst's performance changes little between one and two function executions, since we add a negligible overhead for composing functions.
Lambda, 5$\times$ slower for the stateless invocation and 10$\times$ for composition, increases its latency linearly with the number of functions even when the functions do little computation.
\\}

\review{\noindent \textbf{R3.} The authors should discuss the overheads of tracking dependencies to ensure causal consistency. (W4)\\}

\response{\noindent 
To highlight these overheads, we added an analysis of the per-key causal metadata storage overhead in Section~\ref{sec:eval-consistency}.
Overall, the overhead is modest in our workload, with a median overhead of 624 bytes and a 99-th percentile overhead of 7.1KB.
Although not a focus of this paper, there are techniques that reduces the size of causal metadata such as vector clock compression~\cite{akbar2017icant} and dependency garbage collection~\cite{COPS}, which we plan to explore in future work.
\\}

\review{\noindent \textbf{R4.} The authors should expand their discussion on function scheduling and elasticity. Does more need to occur than copying data from Anna? (D1)\\}

\response{\noindent 
\system{} uses Kubernetes to manage physical resources and to scale the cluster up and down.
As we discuss in Section~\ref{sec:conclusion}, there are potential techniques to improve the responsiveness of \system{} to elasticity which we plan to explore in the future.
With regards to the startup process for each node, the answer is yes---a new node reads data and metadata from Anna to correctly configure itself. 
We have expanded on both these points in Section~\ref{sec:arch-fluent-mgmt}.
\\}

\review{\noindent \textbf{R5.} The authors should enhance the discussion on atomicity and isolation, in particular, the semantics within a DAG. (D2)\\}

\response{\noindent 
Existing FaaS platforms do not have a notion of atomicity or isolation, as we discuss in Section~\ref{sec:motiv-pain}. 
Since they are purely stateless, they do not concern themselves with the semantics of state updates---users are free to use strongly or weakly consistent systems based on their application needs.
Standard serverless storage (e.g., AWS S3 or DynamoDB), however, does not offer strong isolation or fault-tolerance by default.
Our approach, on the other hand, provides coordination-free consistency in the form of repeatable reads and causal consistency for individual DAGs.
\\}

% Nonetheless, we agree that atomicity and other isolation techniques are interesting direction to further explore for stateful serverless infrastructure, but we believe they warrant exploration in separate research. \jmh{I'm not sure how this paragraph helps actually.}
% \chenggang{missing we have clarified this in section xxx.}

\review{\noindent \textbf{R6.} The authors should specify the consistency chosen for the prediction serving workload. (D3)\\}

\response{\noindent 
Thanks for pointing out this omission.
Since the prediction serving workload does not involve concurrent modification to shared state, Cloudburst's default consistency model (last writer wins) is sufficient.
We have clarified this point in Section~\ref{sec:eval-serving}.
\\}

\review{\noindent \textbf{R7.} The authors should clarify how functions can communicate with each other, given the DAG nature of functions. (D4)\\}

\response{\noindent 
We have expanded on the mechanisms for function-to-function communication in Section~\ref{sec:programming}. 
The expected behavior is that functions will broadcast their ID to a pre-agreed upon key in the KVS. 
Another function will read that key and send a message to it, including its own ID as a part of the message.
Once both functions have each others' IDs, they can communicate directly via TCP.
In the case of failure, each executor thread has a KVS key that serves as its inbox, which it periodically reads to ensure it has not missed any messages.

This communication is \emph{not} limited to DAGs---the mechanisms we describe work for non-DAG executions as well.
In fact, the experiment in Section~\ref{sec:eval-comm} does not use DAGs but uses individual function invocations.
\\}

\review{\noindent \textbf{R8.} Address W2.\\}

\response{\noindent 
We concur that mechanisms for serverless infrastructure (e.g. the development of micro-VMs like Firecracker with sub-second startup) are sometimes motivated by challenges of policy (e.g. the inability to make workload predictions on the order of minutes). 
However, the core mechanisms of elasticity are really quite simple: the allocation and deallocation of VMs.
The policies of course need to consider both the infrastructure and workload. 
This includes the time it takes to spin up a node, the ability to predict demand curves in advance, and so on. 
We have clarified this in Section~\ref{sec:arch-fluent-mgmt}.

In our experience, the APIs for elasticity and scheduling are simple enough that we have been able to prototype a range of innovative policies, including Reinforcement Learning policies for elasticity, as well as recently-published scheduling policies like HEFT~\cite{heft}.
We do not yet have results justifying such innovative schemes, and view that as future work outside the scope of the paper. 
\\}

\begin{LARGE}
\textbf{\\ Response to Reviewer 3 \\}
\end{LARGE}

\review{\noindent \textbf{R1.} Contrast ideas better to existing solutions (D1 and D5). \\}

\response{\noindent 
Thanks for pointing out these omissions.
We've included them in our related work section, and we have also cited foundational work related to our architecture in a survey from Franklin and Carey~\cite{franklin1992client}.
\\ }

\review{\noindent \textbf{R2.} Add missing details for core contributions (D4 and D6). \\}

\review{\noindent \textbf{D4.} The caching strategy seems not to scale to a large number of function executors. I am not seeing how maintaining an index on the KV side and propagating key updates to caches can scale to large deployments. \\}

\response{\noindent 
Thanks for this question.
Anna incrementally maintains an index that maps from keys to function executor nodes that cache the keys.
This index is partitioned in Anna by key value---i.e. the index info about each key is stored on the same node as the key itself.
Therefore, we can view the index overhead as a form of per-key metadata storage overhead.
Anna monitors the data and metadata overhead and scales its deployment appropriately.

To quantify this overhead concretely, we revised our autoscaling experiment in Section~\ref{sec:eval-scaling}. 
We benchmark Cloudburst against a moderately contended workload with Zipfian coefficient set to 1.0 and scale the function execution layer to 120 nodes.
Overall, the index overhead is manageable: for keys in our working set, the median index overhead is 24 bytes and the 99-th percentile overhead is 1.3KB, corresponding to keys being cached at 1.6\% and 93\% of the function nodes, respectively.
%In each storage node, we maintain a replica of the index that maps from keys to function executor nodes that cache the keys.
%Therefore, the asymptotic storage overhead of the index is $O(num\_distinct\_keys\_cached * num\_caches)$.
%In our current implementation, each function executor node caches the top 1000 most popular keys and uses LRU policy for eviction (Section~\ref{sec:eval}).
%In our revised autoscaling experiment in Section~\ref{sec:eval-scaling}, we benchmark Cloudburst against a moderately contended workload (with Zipfian coefficient set to 1.0) and scale the function execution layer to 120 nodes.

Propagation of updates from Anna to caches is done periodically in the background and we do not observe significant overhead as Cloudburst autoscales from 60 function nodes to 120.
Further increasing the number of function executors can lead to a larger per-key index size, making the list of matching nodes per key longer and the overhead more pronounced. 
In that case we believe there are opportunities for significant compression to assist with storage and propagation, consistent with prior work on index compression (e.g., bitmap indexes). 
This is out of scope for this paper, but we plan to investigate it in future work. \\ 
}

\review{\noindent \textbf{D6.} Since the distributed consistency schemes are a major contribution of the paper, I would have expected a more thorough presentation of how this is implemented For example, how are timestamps generated? What is the format? How is a version found using timestamps? This should be defined more formally. Moreover, it is not clear how global timestamps are generated in a scalable manner. The paper simply says that it relies on Anna but it is not clear if a severe bottleneck is introduced here. \\}

\response{\noindent 
At each node, a globally-unique timestamp is generated in a standard, scalable, and coordination-free fashion by concatenating the local system clock and the node's unique id.
Timestamps are used in Cloudburst's default last writer wins (LWW) consistency model and repeatable read (RR) consistency model.

In all of our schemes, there is one, up-to-date version of each key in any given cache and one version in Anna.
Under LWW consistency, the lattice merge logic keeps the value with the higher timestamp.
In repeatable read mode, upstream function creates \textit{temporary} snapshots of key versions read in case these versions are later requested by a downstream function---these versions are only visible to functions within the same request. 
These snapshots are garbage collected once the DAG finishes execution.
We have clarified these points as well as the format of the metadata used for causal consistency (vector clocks and dependency sets) in Section~\ref{sec:consistency}.
\\ }

\review{\noindent \textbf{R3.} Show scalability of CloudBurst to larger deployments (D8, D9, and D10) and add other missing details (D7). \\}

\review{\noindent \textbf{D7.} What was the exact setup in Section 6.1.1 and 6.1.3? Was the data store local on the same node as the function executor? How many nodes were used for function executors in 6.1.3? \\}

\response{\noindent 
We have clarified the number of executors and threads used in these experiments.
There was no external data involved in either experiment---requests were passed in from a client, and data was passed between functions (as results in Section~\ref{sec:eval-compostition} and as messages in Section~\ref{sec:eval-comm}).
\\ }

\review{\noindent \textbf{D8.} The caching overhead should be evaluated more thoroughly in 6.1. Does the design which keeps track of items in the caches using a KV-side index scale with the number of function executors? How does the overhead grow then?\\}

\response{\noindent 
Please see our response to D4.
\\ }

\review{\noindent \textbf{D9.} The autoscaling experiments in 6.1.4 is not convincing. I would have expected to see the behavior when scaling to much larger deployments since this is one of the main selling points of CloudBurst.\\}

\response{\noindent 
Thanks for this suggestion.
We increased the scale of our autoscaling experiment by 6$\times$ to 120 function execution nodes, and increased the number of clients by 8$\times$ to 400 concurrent client threads.
We also made the workload stateful: each function reads from two keys and writes to one key drawn from a Zipfian distribution of coefficient 1.0 to measure the overhead of cached key index stored in the KVS.
As discussed in our response to D4 and Section~\ref{sec:eval-scaling}, at this scale, we still observe linear scaling as the system adds in more nodes, and the overhead of the index is not significant.
Further increasing the scale could help us identify more potential bottlenecks; however, due to budget constraints, we did not attempt to run experiments that involve 1000+ nodes (i.e., 3000+ threads)---running the experiment at the current scale on AWS already cost \$2000.
\\ }

\review{\noindent \textbf{D10.} In 6.2 and 6.3 most experiments do not report the size of the deployment. For the distributed consistency protocols, it would be important to show that the protocols scale with the number of function executor AND clients. Same holds for the use cases.\\}

\response{\noindent 
Thanks. We highlighted the deployment sizes and numbers of clients in all of these experiments.
Note that both of our distributed consistency protocols are coordination-free; the overhead of the protocols is orthogonal to the system's deployment size.
For example, in distributed session causal consistency, we guarantee that the key versions read within a DAG satisfy the causal consistency invariant.
To achieve this, only caches involved in the DAG execution must communicate to guarantee that functions read the correct version of keys (Algorithm~\ref{alg:cc}); no global coordination is required.

With these properties and also due to cloud budget limits, we kept the scale of these experiments as-is and focused on a large-scale evaluation (both in the number of function executors and benchmark clients) in Section~\ref{sec:eval-scaling}.
\\ }

\begin{LARGE}
\textbf{\\ Response to Reviewer 5 \\}
\end{LARGE}

\review{\noindent \textbf{R1.} More discussion of how message passing works and its semantics. \\}

\response{\noindent 
We have expanded on the mechanisms and behaviors for message passing in Section~\ref{sec:programming}.
Please see our response to Reviewer 2 R7 from above for a summary of the changes we made.
\\ }

\review{\noindent \textbf{R2.} More discussion of how the causal consistency algorithm works. \\}

\review{\noindent \textbf{D5.} The causal consistency is a bit more interesting, since the technique is to take an existing idea (bolt-on causal consistency) and augment it to have a global causal cut. I would have liked to learn more about this piece. Also, I could not understand from the description how it handles all cases. For example, imagine function F calls function G and function H, and both function G and H read data item X. How does this protocol make sure G and H read the same version of X? The description talks about upstream and downstream nodes sharing vectors of versions, but what about sibling nodes?
\\}

\response{\noindent 
We have clarified the definition of causal consistency in Section~\ref{sec:consistency-guarantees}.
Note that the scenario you pose is considered ``concurrent'' in the definition of causal consistency.
That means $g$ and $h$ may read different versions of $x$, and causal consistency does not specify which of these versions is preferred.
In addition to the clarification above, we have also added more detail about the structure of the causal metadata and the merge logic used by the causal lattice in Section~\ref{sec:consistency-lattice}; we also expanded the explanation of the causal consistency algorithm in Section~\ref{sec:consistency-protocols}.
\\}

%With regard to your question about causal consistency for sibling functions: causal consistency imposes restriction on key versions read between events that have a strict ordering.
%In our context, this means keys read in upstream versus downstream functions, or keys read within the same function.
%Causal consistency does not restrict key versions read by two concurrent events, so key versions read by sibling functions are not required to satisfy the consistency invariant.
%We have made this clarification in Section~\ref{sec:consistency-guarantees}.
%There is a stronger form of causal consistency, called transactional causal consistency (TCC), that guarantees causality for a group of keys read within a transaction (a DAG in our context) regardless of the ordering in which the keys are read.
%In our upcoming SIGMOD'20 paper (http://cgwu.io/files/papers/hydrocache.pdf), we discuss in depth how to support TCC in Cloudburst, which requires new algorithms, and we encourage you to take a look.

\review{\noindent \textbf{R3.} More discussion of which of these changes existing platforms can't support versus which changes they just didn't get around to yet or decided to leave out in the name of simplicity. \\}

\response{\noindent 
Thanks for highlighting this.
Our goal is not to say that the designers of AWS Lambda are incapable of building a stateful serverless system.
Rather, we are interested in exploring the design space of serverless infrastructure and illustrating that it is possible to achieve performant, stateful programming.
We clarified our goals in the introduction.

It would be possible to extend a system like Lambda to support the same semantics as Cloudburst.
However, as we highlight in Sections~\ref{sec:arch} and~\ref{sec:consistency}, there are non-trivial concerns in managing stateful programming and distributed state consistency.
Without knowing the details of Lambda's internals, we believe it's likely that supporting such semantics would require significant architectural changes.
\\}

\review{\noindent \textbf{R4.} Feel free to cut/reduce discussion of autoscaling, repeatable reads, last-writer-wins to make room for the above. \\}

\response{\noindent 
We replaced the old autoscaling experiment with a larger-scale experiment that included a stateful workload (Section~\ref{sec:eval-scaling}).
The only content we removed was a brief related work discussion of distributed Python execution. 
We were able to keep the remaining technical content in the paper while accommodating the changes suggested.
Thanks again for all your feedback.
\\ }
